SafetyBench: Evaluating the Safety of Large Language Models

With the rapid development of Large Language Models (LLMs), increasing attention has been paid to their safety concerns. Consequently, evaluating the safety of LLMs has become an essential task for facilitating the broad applications of LLMs. Nevertheless, the absence of comprehensive safety evaluation benchmarks poses a significant impediment to effectively assess and enhance the safety of LLMs. In this work, we present SafetyBench, a comprehensive benchmark for evaluating the safety of LLMs, which comprises 11,435 diverse multiple choice questions spanning across 7 distinct categories of safety concerns. Notably, SafetyBench also incorporates both Chinese and English data, facilitating the evaluation in both languages. Our extensive tests over 25 popular Chinese and English LLMs in both zero-shot and few-shot settings reveal a substantial performance advantage for GPT-4 over its counterparts, and there is still significant room for improving the safety of current LLMs. We also demonstrate that the measured safety understanding abilities in SafetyBench are correlated with safety generation abilities. Data and evaluation guidelines are available at \url{https://github.com/thu-coai/SafetyBench}{https://github.com/thu-coai/SafetyBench}. Submission entrance and leaderboard are available at \url{https://llmbench.ai/safety}{https://llmbench.ai/safety}.

==> tables/zhsubset_res.tex <==
\begin{table*}[!t]
    \centering
    \footnotesize
    \setlength{\tabcolsep}{4.5pt}
    \renewcommand{\arraystretch}{1.0}
    \begin{tabular}{l|c|ccccccc}
    \toprule
    \textbf{Model} & \textbf{Avg.} & \textbf{OFF} & \textbf{UB} & 
    \textbf{PH} & \textbf{MH} & \textbf{IA} & \textbf{EM} & \textbf{PP} \\
    \midrule
    
    \texttt{Random} & 36.0 & 48.9 & 49.8 & 35.1 & 28.3 & 26.0 & 36.0& 27.8 \\
    \midrule
    \texttt{GPT-4} & 89.7 & 87.7 & 73.3 & 96.7 & 93.0 & 93.3 & 92.7& 91.3\\
    \texttt{ChatGLM2}\begin{CJK}{UTF8}{gbsn}（智谱清言）\end{CJK} & 86.8 & 83.7 & 66.3 & 92.3 & 94.3 & 92.3 & 88.7& 89.7\\
    \texttt{ErnieBot\begin{CJK}{UTF8}{gbsn}（文心一言）\end{CJK}} & 79.0 & 67.3 & 55.3 & 85.7 & 92.0 & 86.7 & 83.0& 83.3\\
    \texttt{internlm-chat-7B} & 78.8 & 76.0 & 65.7 & 78.7 & 87.7 & 82.7 & 81.0 & 80.0 \\
    \texttt{gpt-3.5-turbo} & 78.2 & 78.0 & 70.7 & 70.3 & 86.7 & 84.3 & 73.0& 84.3\\
    \texttt{internlm-chat-7B-v1.1} & 78.1 & 68.3 & 70.0 & 74.7 & 88.3 & 86.7 & 79.3& 79.3\\
    \texttt{Baichuan2-chat-13B} & 78.0 & 68.3 & 62.3 & 78.3 & 89.3 & 87.0 & 77.7& 82.7\\
    \texttt{text-davinci-003} & 77.2 & 65.0 & 56.0 & 82.3 & 88.7 & 86.0 & 77.3& 85.3\\
    \texttt{Baichuan-chat-13B} & 77.1 & 74.3 & 73.0 & 68.7 & 86.3 & 83.0 & 75.3& 79.0\\
    \texttt{Qwen\begin{CJK}{UTF8}{gbsn}（通义千问）\end{CJK}} & 76.9 & 64.5 & 67.6 & 70.1 & 92.1 & 89.4 & 73.9& 81.5\\
    \texttt{ChatGLM2-lite} & 76.1 & 67.0 & 61.3 & 74.0 & 90.0 & 80.7 & 78.7& 81.0\\
    \texttt{ChatGLM2-6B} & 74.2 & 66.7 & 67.0 & 67.7 & 84.7 & 81.3 & 74.3& 78.0\\
    \texttt{Qwen-chat-7B} & 71.9 & 57.0 & 51.0 & 68.7 & 87.3 & 84.0 & 74.7& 80.7\\
    \texttt{SparkDesk\begin{CJK}{UTF8}{gbsn}（讯飞星火）\end{CJK}} & - & 40.7 & - & 57.3 & 83.7 & - & 73.3& 76.7\\
    \texttt{Llama2-Chinese-chat-13B} & 66.4 & 57.7 & 68.7 & 57.7 & 78.3 & 72.0 & 58.7& 71.7\\
    \texttt{Llama2-Chinese-chat-7B} & 59.8& 56.3& 68.7 & 52.7 & 64.3& 60.7 & 49.7& 66.0 \\
    \bottomrule
    \end{tabular}
    
    \caption{Five-shot evaluation results on the filtered Chinese subset of  SafetyBench. ``Avg.'' measures the micro-average accuracy. ``OFF'' stands for \textit{Offensiveness}. ``UB'' stands for \textit{Unfairness and Bias}. ``PH'' stands for \textit{Physical Health}. ``MH'' stands for \textit{Mental Health}. ``IA'' stands for \textit{Illegal Activities}. ``EM'' stands for \textit{Ethics and Morality}. ``PP'' stands for \textit{Privacy and Property}. ``-'' indicates that the model refuses to answer the questions due to the online safety filtering mechanism.} 
    \label{tab:zhsubset_res}
\end{table*}
